Scattering GCN: Overcoming Oversmoothness in Graph Convolutional Networks

Graph convolutional networks (GCNs) have shown promising results in processing graph data by extracting structure-aware features. This gave rise to extensive work in geometric deep learning, focusing on designing network architectures that ensure neuron activations conform to regularity patterns within the input graph. However, in most cases the graph structure is only accounted for by considering the similarity of activations between adjacent nodes, which limits the capabilities of such methods to discriminate between nodes in a graph. Here, we propose to augment conventional GCNs with geometric scattering transforms and residual convolutions. The former enables band-pass filtering of graph signals, thus alleviating the so-called oversmoothing often encountered in GCNs, while the latter is introduced to clear the resulting features of high-frequency noise. We establish the advantages of the presented Scattering GCN with both theoretical results establishing the complementary benefits of scattering and GCN features, as well as experimental results showing the benefits of our method compared to leading graph neural networks for semi-supervised node classification, including the recently proposed GAT network that typically alleviates oversmoothing using graph attention mechanisms.

==> NeurIPS/theory_updated.tex <==
\section{Additional Information Introduced by Node-level Scattering Features}\label{sect_theory}
Before empirically verifying the viability of the proposed architecture in node classification tasks, we first discuss and demonstrate the additional information provided by scattering channels beyond that provided by traditional GCN channels. We first consider information carried by node features, treated as graph signals, and in particular their regularity over the graph. As discussed in Sec.~\ref{sect_graph conv. net}, such regularity is traditionally considered only via smoothness of signals over the graph, as only low frequencies are retained by (local) smoothing operations.
Band-pass filtering, on the other hand, can retain other forms of regularity such as periodic or harmonic patterns. The following lemma demonstrates this difference between GCN and scattering channels.

\begin{lem}\label{thm_Lemma 1}
Let $G_{cyc}^{2n}$ be a cyclic graph on $2n$ nodes, $n\in\mathbb{N}$, and let $\boldsymbol{x}\in\mathbb{R}^{2n}$ be a 2-periodic signal on it (i.e., $\boldsymbol{x}_{2\ell-1}=a$ and $\boldsymbol{x}_{2\ell}=b$, for $\ell\in[n]$ for some $a \neq b \in \mathbb{R}$). Then, for any $\theta \in \mathbb{R}$, the GCN filtering $\boldsymbol{g}_\theta \star \boldsymbol{x}$ from Eq.~\ref{eq_conv. parametrization} yields a constant signal, while the scattering filter $\boldsymbol{\Psi}_0 \boldsymbol{x}$ from Eq.~\ref{eq_wavelet matrix} still produces a 2-periodic signal. Further, this result extends to any finite linear cascade of such filters (i.e., $\boldsymbol{g}_\theta \star \cdots \star \boldsymbol{g}_\theta \star \boldsymbol{x}$ or $\boldsymbol{\Psi}_0 \cdots \boldsymbol{\Psi}_0 \boldsymbol{x}$ with $k\in\mathbb{N}$ filter applications in each).
% it holds for all $k\in\mathbb{N}$ that
% $ %\begin{equation*}
%     \boldsymbol{A}^k \boldsymbol{x} = \frac{a+b}{2} \cdot \ones_{2n},
% $ % \end{equation*}
% produces a constant signal, while
% $ % \begin{equation*}
%     \boldsymbol{\Psi}_0 \boldsymbol{x} = (\Id_n - \boldsymbol{P}) \boldsymbol{x}
%     = \boldsymbol{x} - \frac{a+b}{2} \cdot \ones_{2n}
%     = \boldsymbol{x} - \overline{\boldsymbol{x}} \cdot \ones_{2n}
% $ % \end{equation*}
% is still 2-periodic.
\end{lem}
%
While this is only a simple example, it already indicates a fundamental difference between the regularity patterns considered in graph convolutions compared to our approach. Indeed, it implies that if a smoothing convolutional filter encounters alternating signals on isolated cyclic substructures within a graph, their node features become indistinguishable, while scattering channels (with appropriate scales, weights and bias terms) will be able to make this distinction. Moreover, this difference can be generalized further beyond cyclic structures to consider features encoding two-coloring information on constant-degree bipartite graphs, as shown in the following lemma. We refer the reader to the supplement for a proof of this lemma, which also covers the previous one as a particular case.
%
\begin{lem}\label{thm_Lemma 2}
Let $G_{bi, \beta}^n$ be a bipartite graph on $n\in\mathbb{N}$ nodes with constant node degree $\beta$. Let $\boldsymbol{x}\in\mathbb{R}^{n}$ be a 2-coloring signal (i.e., with one part assigned constant $a$ and the other $b$, for some $a \neq b \in \mathbb{R}$). Then, for any $\theta \in \mathbb{R}$, the GCN filtering $\boldsymbol{g}_\theta \star \boldsymbol{x}$ from Eq.~\ref{eq_conv. parametrization} yields a constant signal, while the scattering filter $\boldsymbol{\Psi}_0 \boldsymbol{x}$  from Eq.~\ref{eq_wavelet matrix} still produces a (non-constant) 2-coloring of the graph. Further, this result extends to any finite linear cascade of such filters (i.e., $\boldsymbol{g}_\theta \star \cdots \star \boldsymbol{g}_\theta \star \boldsymbol{x}$ or $\boldsymbol{\Psi}_0 \cdots \boldsymbol{\Psi}_0 \boldsymbol{x}$ with $k\in\mathbb{N}$ filter applications in each).
\end{lem}

% \begin{figure}
% \centering
% \subfigure[Filter response of $\boldsymbol{g}_\theta \star \boldsymbol{x}$]{\label{fig_toy example GCN}
% \adjustbox{width=0.45\textwidth}{\begin{tikzpicture}
%     \node[shape=circle,draw=black, fill=black!50!green] (0) at (0,0) {};
%     \node[shape=circle,draw=black, fill=black!50!green] (1) at (0.6,0.6) {};
%     \node[shape=circle,draw=black, fill=brown] (2) at (1.6,0.6) {};
%     \node[shape=circle,draw=black, fill=black] (3) at (2.2,0) {};
%     \node[shape=circle,draw=black, fill=brown] (4) at (1.6,-0.6) {};
%     \node[shape=circle,draw=black, fill=black!50!green] (5) at (0.6,-0.6) {};
    
%     \node[shape=circle,draw=black, fill=black] (6) at (3.2,0) {};
%     \node[shape=circle,draw=black, fill=brown] (7) at (3.8,0.6) {};
%     \node[shape=circle,draw=black, fill=black!50!green] (8) at (4.8,0.6) {};
%     \node[shape=circle,draw=black, fill=black!50!green] (9) at (5.8,0.6) {};
%     \node[shape=circle,draw=black, fill=black!50!green] (10) at (6.4,0) {};
%     \node[shape=circle,draw=black, fill=black!50!green] (11) at (5.8,-0.6) {};
%     \node[shape=circle,draw=black, fill=black!50!green] (12) at (4.8,-0.6) {};
%     \node[shape=circle,draw=black, fill=brown] (13) at (3.8,-0.6) {};

%     \path [-] (0) edge (1);
%     \path [-] (1) edge (2);
%     \path [-] (2) edge (3);
%     \path [-] (3) edge (4);
%     \path [-] (4) edge (5);
%     \path [-] (5) edge (0);
    
%     \path [-] (3) edge (6);
%     \path [-] (6) edge (7);
%     \path [-] (7) edge (8);
%     \path [-] (8) edge (9);
%     \path [-] (9) edge (10);
%     \path [-] (10) edge (11);
%     \path [-] (11) edge (12);
%     \path [-] (12) edge (13);
%     \path [-] (13) edge (6);
% \end{tikzpicture}}}
% \quad
% \subfigure[Filter response of $\boldsymbol{\Psi}_3 \boldsymbol{x}$]{\label{fig_toy example scat}
% \adjustbox{width=0.45\textwidth}{\begin{tikzpicture}
%     \node[shape=circle,draw=black, fill=black!20!green] (0) at (0,0) {};
%     \node[shape=circle,draw=black, fill=black!60!green] (1) at (0.6,0.6) {};
%     \node[shape=circle,draw=black, fill=blue] (2) at (1.6,0.6) {};
%     \node[shape=circle,draw=black, fill=white!70!blue] (3) at (2.2,0) {};
%     \node[shape=circle,draw=black, fill=blue] (4) at (1.6,-0.6) {};
%     \node[shape=circle,draw=black, fill=black!60!green] (5) at (0.6,-0.6) {};
    
%     \node[shape=circle,draw=black, fill=white!90!black] (6) at (3.2,0) {};
%     \node[shape=circle,draw=black, fill=white!60!black] (7) at (3.8,0.6) {};
%     \node[shape=circle,draw=black, fill=black] (8) at (4.8,0.6) {};
%     \node[shape=circle,draw=black, fill=brown] (9) at (5.8,0.6) {};
%     \node[shape=circle,draw=black, fill=white!50!brown] (10) at (6.4,0) {};
%     \node[shape=circle,draw=black, fill=brown] (11) at (5.8,-0.6) {};
%     \node[shape=circle,draw=black, fill=black] (12) at (4.8,-0.6) {};
%     \node[shape=circle,draw=black, fill=white!60!black] (13) at (3.8,-0.6) {};

%     \path [-] (0) edge (1);
%     \path [-] (1) edge (2);
%     \path [-] (2) edge (3);
%     \path [-] (3) edge (4);
%     \path [-] (4) edge (5);
%     \path [-] (5) edge (0);
    
%     \path [-] (3) edge (6);
%     \path [-] (6) edge (7);
%     \path [-] (7) edge (8);
%     \path [-] (8) edge (9);
%     \path [-] (9) edge (10);
%     \path [-] (10) edge (11);
%     \path [-] (11) edge (12);
%     \path [-] (12) edge (13);
%     \path [-] (13) edge (6);
% \end{tikzpicture}}}
% \caption{Filter responses for \subref{fig_toy example GCN} the GCN filter from Eq.~\ref{eq_conv. parametrization} and \subref{fig_toy example scat} a scattering-channel filter, when applied to a constant signal $\boldsymbol{x}$ over a graph with two cyclic substuctures connected by a single-edge bottleneck. Color coding differs slightly between plots, but is consistent within each plot, indicating nodes with numerically indistinguishable response values.}
% \label{fig: toy example}
% \end{figure}

\begin{figure}
\centering
\subfigure[Filter response of $\boldsymbol{g}_\theta \star \boldsymbol{x}$]{\label{fig_toy example GCN}
\begin{minipage}{0.45\columnwidth}
\centering
\begin{tikzpicture}[scale=0.9]
    \node[shape=circle,draw=black, fill=blue!50!white] (0) at (0,0) {};
    \node[shape=circle,draw=black, fill=blue!50!white] (1) at (0.6,0.6) {};
    \node[shape=circle,draw=black, fill=blue!10!white] (2) at (1.6,0.6) {};
    \node[shape=circle,draw=black, fill=black!10!blue] (3) at (2.2,0) {};
    \node[shape=circle,draw=black, fill=blue!10!white] (4) at (1.6,-0.6) {};
    \node[shape=circle,draw=black, fill=blue!50!white] (5) at (0.6,-0.6) {};
    
    \node[shape=circle,draw=black, fill=black!10!blue] (6) at (3.2,0) {};
    \node[shape=circle,draw=black, fill=blue!10!white] (7) at (3.8,0.6) {};
    \node[shape=circle,draw=black, fill=blue!50!white] (8) at (4.8,0.6) {};
    \node[shape=circle,draw=black, fill=blue!50!white] (9) at (5.8,0.6) {};
    \node[shape=circle,draw=black, fill=blue!50!white] (10) at (6.4,0) {};
    \node[shape=circle,draw=black, fill=blue!50!white] (11) at (5.8,-0.6) {};
    \node[shape=circle,draw=black, fill=blue!50!white] (12) at (4.8,-0.6) {};
    \node[shape=circle,draw=black, fill=blue!10!white] (13) at (3.8,-0.6) {};

    \path [-] (0) edge (1);
    \path [-] (1) edge (2);
    \path [-] (2) edge (3);
    \path [-] (3) edge (4);
    \path [-] (4) edge (5);
    \path [-] (5) edge (0);
    
    \path [-] (3) edge (6);
    \path [-] (6) edge (7);
    \path [-] (7) edge (8);
    \path [-] (8) edge (9);
    \path [-] (9) edge (10);
    \path [-] (10) edge (11);
    \path [-] (11) edge (12);
    \path [-] (12) edge (13);
    \path [-] (13) edge (6);
\end{tikzpicture}
\end{minipage}
}
\quad
\subfigure[Filter response of $\boldsymbol{\Psi}_3 \boldsymbol{x}$]{\label{fig_toy example scat}
\begin{minipage}{0.45\columnwidth}
\centering
\begin{tikzpicture}[scale=0.9]
    \node[shape=circle,draw=black, fill=white!70!yellow] (0) at (0,0) {};
    \node[shape=circle,draw=black, fill=yellow!90!red] (1) at (0.6,0.6) {};
    \node[shape=circle,draw=black, fill=red] (2) at (1.6,0.6) {};
    \node[shape=circle,draw=black, fill=black!40!red] (3) at (2.2,0) {};
    \node[shape=circle,draw=black, fill=red] (4) at (1.6,-0.6) {};
    \node[shape=circle,draw=black, fill=yellow!90!red] (5) at (0.6,-0.6) {};
    
    \node[shape=circle,draw=black, fill=black!70!red] (6) at (3.2,0) {};
    \node[shape=circle,draw=black, fill=black!20!red] (7) at (3.8,0.6) {};
    \node[shape=circle,draw=black, fill=yellow!20!red] (8) at (4.8,0.6) {};
    \node[shape=circle,draw=black, fill=yellow!60!red] (9) at (5.8,0.6) {};
    \node[shape=circle,draw=black, fill=yellow!40!red] (10) at (6.4,0) {};
    \node[shape=circle,draw=black, fill=yellow!60!red] (11) at (5.8,-0.6) {};
    \node[shape=circle,draw=black, fill=yellow!20!red] (12) at (4.8,-0.6) {};
    \node[shape=circle,draw=black, fill=black!20!red] (13) at (3.8,-0.6) {};

    \path [-] (0) edge (1);
    \path [-] (1) edge (2);
    \path [-] (2) edge (3);
    \path [-] (3) edge (4);
    \path [-] (4) edge (5);
    \path [-] (5) edge (0);
    
    \path [-] (3) edge (6);
    \path [-] (6) edge (7);
    \path [-] (7) edge (8);
    \path [-] (8) edge (9);
    \path [-] (9) edge (10);
    \path [-] (10) edge (11);
    \path [-] (11) edge (12);
    \path [-] (12) edge (13);
    \path [-] (13) edge (6);
\end{tikzpicture}
\end{minipage}
}
\caption{Filter responses for \subref{fig_toy example GCN} the GCN filter from Eq.~\ref{eq_conv. parametrization} and \subref{fig_toy example scat} a scattering channel filter when applied to a constant signal $\boldsymbol{x}$ over a graph with two cyclic substuctures connected by a single-edge bottleneck. The color coding indicates nodes with numerically indistinguishable filter responses.}
\label{fig: toy example}
\end{figure}

Beyond the information encoded in node features, graph wavelets can be shown to encode geometric information even when it is not carried by input signals. Such a property has already been established, for example, in the context of community detection, where white noise signals can be used in conjunction with graph wavelets to cluster nodes and reveal faithful community structures~\citep{roddenberry2020exact}.
To demonstrate a similar property in the context of GCN and scattering channels, we give an example of a simple graph structure with two cyclic substructures of different sizes (or cycle lengths) that are connected by one bottleneck edge. In this case, it can be verified that even with constant input signals, some geometric information will be encoded by its convolution with graph filters, as illustrated in Fig.~\ref{fig: toy example} (we refer the reader to the supplement for exact calculation of filter responses). However, as demonstrated in this case, while the information provided by the GCN filter responses $\boldsymbol{g}_\theta \star \boldsymbol{x}$ from Eq.~\ref{eq_conv. parametrization} is not constant, it does not distinguish between the two cyclic structures in the graph (and a similar pattern can be verified for $\boldsymbol{Ax}$). Formally, each node $u$ in one cycle is shown to have at least one node $v$ in the other with the same filter response (i.e., $\boldsymbol{g}_\theta \star \boldsymbol{x} (u) = \boldsymbol{g}_\theta \star \boldsymbol{x}(v)$). In contrast, the information extracted by the wavelet filter responses $\boldsymbol{\Psi}_3 \boldsymbol{x}$ (e.g., used in Geometric Scattering) does distinguish between cycles, and would allow for their separation. We note that this property generalizes to other cycle lengths, as discussed further in the supplement, but leave more extensive study of geometric information encoding in graph wavelets to future work.






==> arxiv/abstract.tex <==
Graph convolutional networks (GCNs) have shown promising results in processing graph data by extracting structure-aware features. This gave rise to extensive work in geometric deep learning, focusing on designing network architectures that ensure neuron activations conform to regularity patterns within the input graph. However, in most cases the graph structure is only accounted for by considering the similarity of activations between adjacent nodes, which in turn degrades the results. In this work, we augment GCN models by incorporating richer notions of regularity by leveraging cascades of band-pass filters, known as geometric scatterings. The produced graph features incorporate multiscale representations of local graph structures, while avoiding overly smooth activations forced by previous architectures. Moreover, inspired by skip connections used in residual networks, we introduce graph residual convolutions that reduce high-frequency noise caused by joining together information at multiple scales. Our hybrid architecture introduces a new model for semi-supervised learning on graph-structured data, and its potential is demonstrated for node classification tasks on multiple graph datasets, where it outperforms leading GCN models.
